H-\"aquivariante Morita-\"Aquivalenz und Deformationsquantisierung

English abstract: This work contains of five chapters: The first one deals with Morita equivalence of star algebras. In particular star algebras which are equipped with a symmetry given by a Hopf (star-) algebra. In the second chapter we describe the equivariant Picard group and the equivariant Picard groupoid, which are a direct consequence of the results from the first chapter. We calculated the kernel and the image of the groupoid morphism from the equivariant Picard groupoid into the normal one. We give furthermore a formalized version of Morita invariance: given by a functor from the Picard groupoid to another category. This is shown for several examples. In the third chapter we show the connection between Hopf equivariant Morita equivalence of star algebras and the Morita equivalence of cross-product algebras. The forth chapter deals with deformation quantization and gives an extended introduction to (invariant) star products. In the fifth chapter we show the Hopf equivariance of deformed algebras (i.e. of hermitian star products). This is a important examples which concludes the previous chapters.

==> babelbst.tex <==
\newcommand{\bbland}{und}
\newcommand{\bbleditor}{Hrsg.}
\newcommand{\bbleds}{Hrsg.}
\newcommand{\bbledby}{herausgegeben von}
\newcommand{\bbledn}{Auflage}
\newcommand{\bblvol}{Band}
\newcommand{\bblof}{von}
\newcommand{\bblno}{Nr.}
\newcommand{\bblin}{in}
\newcommand{\bblpp}{S.}
\newcommand{\bblp}{S.}
\newcommand{\bblchap}{Kapitel}
\newcommand{\bbltechrep}{Tech.~Rep.}
\newcommand{\bblmthesis}{Diplomarbeit}
\newcommand{\bblphdthesis}{Dissertation}
\newcommand{\bbljan}{Jan}
\newcommand{\bblfeb}{Feb}
\newcommand{\bblmar}{M"ar}
\newcommand{\bblapr}{Apr}
\newcommand{\bblmay}{Mai}
\newcommand{\bbljun}{Jun}
\newcommand{\bbljul}{Jul}
\newcommand{\bblaug}{Aug}
\newcommand{\bblsep}{Sep}
\newcommand{\bbloct}{Okt}
\newcommand{\bblnov}{Nov}
\newcommand{\bbldec}{Dez}
\newcommand{\bbletal}{et al.}
\newcommand{\eprint}{\tt}
\newcommand{\bblvolume}{Vol.}
\newcommand{\bblnumber}{Nr.}
\newcommand{\bbledition}{Auflage}
\newcommand{\bblsecondo}{2.}
\newcommand{\bblthirdo}{3.}
\newcommand{\bblfourtho}{4.}
\newcommand{\bblfourth}{4.}
\newcommand{\bblsecond}{2.}
\newcommand{\bblthird}{3.} 
\newcommand{\bblpages}{S.}
\newcommand{\bblth}{.}

==> gruppen.tex <==
\chapter{Gruppen, \Name{Lie}-Algebren und Aktionen}


\begin{definition}[Gruppe]
Sei $G$ eine Menge mit einer Verkn\"upfung $\mu: G \times G \to G$,
mit den folgenden Eigenschaften.
\begin{compactenum}
    \item Die Verkn\"upfung $\mu$ ist {\em assoziativ}, d.h.~es gilt
        f\"ur alle Elemente $g,h,k \in G$ $\mu(\mu(g,h),k) = \mu(g,
        \mu(h,k))$. 
    \item Es existiert ein {\em Einselement} $e \in G$ so da{\ss}
        f\"ur alle $g \in G$ gilt: $\mu (e,g)=\mu (g,e)=g$.
    \item Zu jedem Element $g\in G$ existiert ein {\em Inverseses}
        $h$, so da{\ss} $\mu(g,h)=\mu(h,g)=e$. Das Inverse des
        Elements $g$ bezeichnet man mit $g^{-1}$.   
\end{compactenum}
Man nennt $(G,\mu)$ eine {\em Gruppe}. 
\end{definition}


\begin{bemerkung}
Die Verkn\"upfung $\mu$ wird von uns meist unterschlagen, was an die
gew\"ohnlichen Multiplikation angelehnt ist. Ist die Gruppe {\em
  \Name{Abel}sch}, 
d.h.~gilt f\"ur alle $g,h \in G$ $\mu(g,h)=\mu(h,g)$, so
kennzeichnen wir die Verkn\"upfung gelegentlich durch $+$. 
\end{bemerkung}





\begin{definition}[Gruppenaktion]
Sei $M$ eine Mannigfaltigkeit. Man nennt eine Gruppenaktion $\phi_{g}
: M \to M$ auf der Mannigfaltigkeit 
\begin{compactenum}
\item {\em frei}, falls
\item {\em eigentlich}, falls
\item {\em }, falls
\end{compactenum}
    
\end{definition}

\begin{definition}[$G$-Mannigfaltigkeit]
 \label{Definition:GMannigfaltigkeit}
 Ein Mannigfaltigkeit $M$ mit einer Gruppenaktion der Gruppe $G$, die
 via einer Linksaktion\footnote{Jede Linksaktion kann ebenso als eine
   Rechtsaktion $\Psi$ aufgefa{\ss}t werden, da $\psi_{g^{-1}} =
   \phi_{g}$. Wir werden uns in dieser Arbeit daher nur auf
   Linksaktionen beschr\"anken.} 
 \begin{align}
     \label{eq:LinksaktionAufMannigfaltigkeit}
     \phi: G \times M \to M,\qquad  (g,m) \mapsto \phi(g,m)=: \phi_{g}
     (m) =g.m
 \end{align}
f\"ur alle $g\in G$ und $m\in M$ auf die Mannigfaltigkeit wirkt,
bezeichnet man als {\em $G$-Mannigfaltigkeit}. Wir bezeichnen
$G$-Mannigfaltigkeiten mit $(M,G)$. 
\end{definition}

Offensicht gilt dann $\phi_{g}\circ \phi_{g'} = \phi_{gg'}$,
$\phi_{e}= \id$ und $\phi_{g}^{-1}=\phi_{g^{-1}}$. 


\begin{definition}[$G$-Vektorb\"undel]
    Sei $\bundle{E}{\pi}{(M,G)}$ ein Vektor\"undel \"uber einer
    $G$-Mannigfaltigkeit. Man nennt das Vektorb\"undel ein {\em
      $G$-Vektorb\"undel}, falls es eine geliftete Gruppenaktion 
\begin{align}
\Phi : G \times E \to E, \qquad (g,v) \mapsto
\Phi(g,v)=:\Phi_{g}(v)=g.v     
\end{align}
gibt, so da{\ss} f\"ur alle $v\in E$ und $g \in G$ gilt $\pi \circ
\Phi = \phi \circ \pi$.  
\end{definition}

\begin{definition}[Symplektomorphismus]
Sei $(M,\omega,G)$ eine symplektische $G$-Mannigfaltigkeit. Die
Linksaktion $\phi_{g}:M \to M$ ist ein {\em Symplektomorphismus} falls
\begin{align}
    \label{eq:Symplektomorphismus}
    \phi_{g}^{\ast} \omega = \omega
\end{align}
f\"ur alle $g \in G$.
\end{definition}




\begin{definition}[Darstellung einer Gruppe]
Gegeben eine Gruppe $G$ und ein $n$-dimensionaler Vektorraum $V$. Eine
{\em Darstellung} der Gruppe $G$ ist ein Homomorphismus $\varrho: G
\to \End(V)$, so da{\ss} $\varrho(gh)=\varrho(g) \varrho(h)$.
\end{definition}





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "dissertation"
%%% End: 

